Bridging the Gap: Automated Analysis of Sancus

Techniques for verifying or invalidating the security of computer systems have come a long way in recent years. Extremely sophisticated tools are available to specify and formally verify the behavior of a system and, at the same time, attack techniques have evolved to the point of questioning the possibility of obtaining adequate levels of security, especially in critical applications. In a recent paper, Bognar et al. have clearly highlighted this inconsistency between the two worlds: on one side, formal verification allows writing irrefutable proofs of the security of a system, on the other side concrete attacks make these proofs waver, exhibiting a gap between models and implementations which is very complex to bridge. In this paper, we propose a new method to reduce this gap in the Sancus embedded security architecture, by exploiting some peculiarities of both approaches. Our technique first extracts a behavioral model by directly interacting with the real Sancus system and then analyzes it to identify attacks and anomalies. Given a threat model, our method either finds attacks in the given threat model or gives probabilistic guarantees on the security of the system. We implement our method and use it to systematically rediscover known attacks and uncover new ones.

==> sections/background.tex <==
% !TEX root = ../main.tex
Automata learning, bisimulation, sancus and enclaved archs


==> sections/discussion.tex <==
% !TeX root = ../main.tex

%Despite not being able to look exhaustively to all the possible attackers, we looked into
We consider possible variations of the attack scenarios presented in \cref{sec:sancus}
using
%the above attacker's capabilities,
%the violation witnesses as a starting point,
%We conducted these tests by specifying variations of our attackers in the usual format and using
%and
the tool to directly execute input traces and inspect the abstract behavior.
% , and the results are drawn directly from the signal dumps produced by the Verilog simulator.
% \ricS{Ma perché a mano? Sembra out-of-scope detto così. Comunque il tool permette di specificare attaccanti specifici right? Immagino tu l'abbia fatto così ...}
% \matteoS{Forse si riesce a fare così...}
The code and scripts to run the examples of this section are also available online~\cite{additionalmaterial}, in the \texttt{spec-lib/extra} folder.


\subsection{Security Under Extended Attackers}
%
% Non molto interessante, e non si capisce perchè uno dovrebbe testarla in effetti
% The first variant we considered has capability \textbf{C3} (i.e., resetting or halting the CPU) inside the \lstinline|isr| section.
% Halting and resetting the machine inside the ISR is allowed both in the formal Sancus model~\cite{busi2021securing} and in the implementation, as we evaluated experimentally using \toolname and one may wonder whether this may rise security issues.
% The additional capability of stopping or resetting the system before the \lstinline|cleanup| does not introduce additional confidentiality and integrity issues.
% \ricS{ma perché questa non è una capability come le altre e va fatta a mano?}
% In fact, when the system is halted, neither the attacker nor the enclave can perform new observations and operations.
% Moreover, when the system resets, its state is cleared so making old registers and memory values inaccessible, trivially forbidding further exploitation.
% \ricS{Quindi? Non si capisce bene cosa vuoi dire qui.}
Inspired by the capabilities of the attackers in~\cref{sec:att-b37}, we have devised a  variant \textbf{C5'} of the standard capability \textbf{C5}.
With \textbf{C5'}, an attacker can make a \lstinline|reti| instruction jump into the middle of an enclave by pushing an enclave's address directly onto the stack.

Executing an abstract trace that uses \textbf{C5'} in the \lstinline|cleanup| section, we found out the following interesting facts. In the first commit of Sancus in~\cite{mindthegap-repo} and up to the commit that fixes attack \textbf{V-B3}, if the \lstinline|reti| is issued after exiting from an enclave, the processor behaves consistently to the \textbf{V-B3} attack: the enclave execution is restored in the middle because the \emph{shadow registers}\footnote{The shadow registers are used to temporarily store the state of the enclave while the \lstinline|isr| is running.} of Sancus are not cleared properly when exiting the \lstinline|isr|.
In any other case, performing the \lstinline|reti| instruction raises an exception, and consequently a reset of the system.
Therefore, the forced return to the code and data sections cannot be exploited by  attackers to carry out new attacks.

We also tested whether it is possible to interrupt the enclave creation process corrupting the system state.
This is modeled as a variant of capability \textbf{C4}, that we call \textbf{C4'}.
\toolname fails to automatically validate this example because it detects a behavior that is not (yet) supported, i.e., the interrupt raised outside the enclave, but the simulator still produces the full VCD file with the dump of all the  signals.
% We used this to validate that the CPU is properly masking interrupts during creating the enclave directly, thus inhibiting our attacker.
We used this to directly validate that the CPU is properly masking interrupts during the creation of the enclave, thus inhibiting our attacker.
% \ricS{Anche questo perché non è modellato come capability?}\matteoS{meglio così?}

\subsection{New Anomalies}
%
Another interesting extension is
%perhaps simpler experiment than the one using the \lstinline|reti| instruction,
the possibility to jump directly to enclave addresses using  \lstinline|jmp|.
This can be modeled as a variant of \textbf{C2}, that we call \textbf{C2'}.
When we executed abstract traces using the   \textbf{C2'} capability in the \lstinline|prepare| section,
% Jumping directly in the middle of an enclave,
we found that the CPU seems to execute \lstinline|jmp| correctly, before raising an exception.
%Inspecting the execution more closely,
We also discovered that the system takes one extra clock cycle before resetting.
Most likely, this is due to the fact that violations are detected when the fetch to a prohibited location occurs, so one clock cycle after \lstinline|jmp|.
% the PC tries to execute in forbidden location.
Interestingly, when the attacker tries to jump into the enclave's data memory initialized with a valid op-code the abstract behavior reports a successful jump followed by an infinite loop of the processor.
%Upon closer inspection,
We also found that the CPU executes code at the destination address indefinitely.
% (even if it takes more than $1$ cycle)\ricS{continuo a non capire la parte tra parentesi}.
Surprisingly though, the value of the program counter also changes and is incremented by the CPU at each clock cycle.


% While these anomalies appear unexploitable in the current model of the Sancus attacker, i.e., one that ignores system availability and lacks persistent storage capabilities, they represent \emph{novel} discrepancies in the model's implementation in the style of those found by ~\citet{mindthegap}.
% Recall that a model implementation is a discrepancy between the formal Sancus model of~\citet{busi2021securing} and the actual architecture implementation.

A final test we conducted using \toolname
%and inspired by these observations
aims to find out whether exceptions occurring inside enclaves lead to attacker-controlled ``cleanup'' code, as it happens in the formal model of Sancus~\cite{busi2021securing}.
%
Notice that, this mechanism gives attackers more power, allowing them to distinguish otherwise indistinguishable enclaves.
%
We discovered that the CPU never gives the control back to the attacker upon violations in the enclave, instead it resets the system.
This anomaly becomes an issue with attackers that have capability \textbf{C4}.
Indeed, suppose that the enclave under attack raises an exception at different times depending on the value of a secret:
% \ricS{Perché questo codice è colored e gli altri no? Li fa stonare .... :)}
%
\lstset{language=msp430asm}
\begin{lstlisting}
      cmp #SECRET, r8        ; if r8 == SECRET
      jnz else
      nop                    ; Waits one cycle
else: mov #1, &unprot_memory ; Raises an exception
\end{lstlisting}
%
% An attacker without \textbf{C4} is not able to learn anything about the value of \lstinline|SECRET|, but
An attacker that schedules an interrupt at the exact time in which \lstinline|nop| should happen is able to discover the result of the \lstinline|cmp| instruction and, consequently, the value of \lstinline|SECRET| by simply detecting whether its \lstinline|isr| is executed or not.

These anomalies are not exploitable by an attacker because, apparently, the temporal behavior has no dependencies on code or data in Sancus, but could be exploitable in a different architecture or in future Sancus extensions. In fact, they represent \emph{novel} discrepancies in the model's implementation in the style of those found by ~\citet{mindthegap}.

% However, note that such discrepancy between the formal model and the implementation does not enable new attacks.
% Indeed, since the architecture cannot forbid crashes inside enclaves, enclaves showing the behavior above must be considered inherently insecure.
% The implementation should be adapted accordingly.\ricS{Non ho capito}

% \matteo{E' strana questa cosa, non so se dirla: nel tool ho messo una flag per abilitare e disabilitare.}
% Finally, we considered an attacker that may use the knowledge from a previous runs to try to attack a system.
% A classical example is the attacker that tries to bruteforce a password: they choose a password, try it and if it is wrong they reboot and try with another, different password.
% We equipped our tool for comparing the models with a special command-line option to allow this behavior in attackers and some variants to the previously-known attacks were discovered.
% For instance, the basic attacker enriched with this capability also carries out the attack whose trace is $...$ that highlights a NI violation when compared to the trace $...$.\ricS{Da completare}

% \subsection{Missing attacks}\flaS{Metterlo  nelle  conclusioni?}\flaS{}
%





==> sections/extra.tex <==
% !TeX root = ../main.tex

\subsection*{Model-implementation mismatches from~\cite{mindthegap}}
%
Since in the following we will focus, among other things, on systematically reproducing the results by~\citet{mindthegap} we summarize here their main discoveries on the Sancus architecture.\matteoS{Da mettere in background o subito prima delle attacker capabilities?}\ricS{Direi qui prima delle attacker capabilities}

In particular they distinguish two classes of discoveries: \emph{implementation-model mismatches} (IMs) and \emph{missing attacker capabilities} (MAs).

IMs identify discrepancies between the Sancus implementation and its formal model, \sancusv~\cite{busi2021securing}, leading to attacks that can be performed on the implementation, but are unsuccessful in the model.
The IM \textbf{V-B1} shows that the first instruction following a \lstinline|reti| takes one additional cycle in the implementation w.r.t.\ what expected in \sancusv.
\textbf{V-B2} identifies an instruction (a \lstinline|mov| between locations in the code memory) that takes $7$ cycles, contrary to the assumption in \sancusv that the maximum duration of instructions is $6$ cycles.
\textbf{V-B3} shows that enclaves can be resumed multiple times using a \lstinline|reti| and \textbf{V-B4} show that restarting an interrupted enclave from the interrupt-service routine is permitted in the implementation.
Both actions are forbidden in \sancusv.
\textbf{V-B5} concerns the possibility of creating multiple enclaves, an action which is not supported by the model.
Finally, \textbf{V-B6} and \textbf{V-B7} show that the access-control policy given by \sancusv is not correctly implemented.

MAs denote instead discrepancies between the actual capabilities of attackers and those modelled in the formal semantics and \citet{mindthegap} identify two such issues, \textbf{V-C1} and \textbf{V-C2}.
The first shows how to exploit unmodelled DMA peripherals to carry out an attack in the Sancus implementation, the second does the same with the unmodelled watchdog timer.

All the IMs and MAs that were found in~\citet{mindthegap} are briefly described and summarized in~\cref{tab:mindthegap}.
For further details, we refer the interested reader to the original paper.
%
\newcommand{\vbonedescr}{The first instruction after a \texttt{reti} takes one additional cycle}
\newcommand{\vbtwodescr}{There exists an instruction with execution time $>6$}
\newcommand{\vbthreedescr}{Enclaves can be resumed multiple times with \lstinline|reti|}
\newcommand{\vbfourdescr}{Restarting an interrupted enclave from the interrupt-service routine is allowed}
\newcommand{\vbfivedescr}{Creation of multiple enclaves is allowed}
\newcommand{\vbsixdescr}{Enclaves can access unprotected memory}
\newcommand{\vbsevendescr}{Enclaves can manipulate interrupt behavior}
\newcommand{\vconedescr}{The formal model misses DMA peripherals}
\newcommand{\vctwodescr}{The formal model misses the watchdog timer}
%
\begin{table}[tb]
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lll@{}}
    \toprule
        % & Name & Discrepancy\\ \midrule
    \multirow{7}{*}{\centering \textbf{IMs}} &
          \textbf{V-B1} & \vbonedescr \\
        & \textbf{V-B2} & \vbtwodescr \\
        & \textbf{V-B3} & \vbthreedescr \\
        & \textbf{V-B4} & \vbfourdescr\\
        & \textbf{V-B5} & \vbfivedescr\\
        & \textbf{V-B6} & \vbsixdescr\\
        & \textbf{V-B7} & \vbsevendescr\\ \midrule
        \multirow{2}{*}{\centering \textbf{MAs}} &
          \textbf{V-C1} & \vconedescr\\
        & \textbf{V-C2} & \vctwodescr\\ \bottomrule
    \end{tabular}
    }

    \caption{\small Summary of IMs and MAs that were discovered by~\citet{mindthegap}.}\label{tab:mindthegap}
\end{table}
%

\subsection*{Big Comment, $1$}

\matteo{Ok per togliere le tracce, i nomi dei commit e dire una volta sola del materiale aggiuntivo.
Le tracce le avevoi messe per dare gli esempi ma non piacevano molto nemmeno a me e i witness graph oltre a non starci sono troppo time consuming da scrivere.
Dove non è molto chiaro }

\subsection*{Performance e hardware}
\matteo{Aggiungere questa frase quando diciamo dell'additional material all'inizio della sezione --- non conosco i dettagli di ciscottone}

Our experiments have been done on a server equipped with an Intel(R) Xeon(R) E5-2699 v4 @ 2.20GHz with 42 CPUs and 128GB of RAM. Running all the experiments described in this section takes about $4$ hours on our machine.
This relatively short learning time comes from the fact that \toolname spawns multiple processes, one for each learning and checking task, making full use of the multicore features of our machine.

\subsection*{Tabellina con tutti i check, non so dove metterla.}

\matteo{Ora la preparo.}


==> witnesses/ef753b6-b3.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (0) at (121.75bp,1669.5bp) [draw,circle] {0};
  \node (1) at (121.75bp,1582.5bp) [draw,circle] {1};
  \node (2) at (121.75bp,1495.5bp) [draw,circle] {2};
  \node (3) at (121.75bp,1408.5bp) [draw,circle] {3};
  \node (4) at (121.75bp,1321.5bp) [draw,circle] {4};
  \node (5) at (121.75bp,1234.5bp) [draw,circle] {5};
  \node (6) at (121.75bp,1147.5bp) [draw,circle] {6};
  \node (7) at (121.75bp,1060.5bp) [draw,circle] {7};
  \node (8) at (121.75bp,973.46bp) [draw,circle] {8};
  \node (9) at (121.75bp,886.46bp) [draw,circle] {9};
  \node (10) at (121.75bp,794.72bp) [draw,circle] {10};
  \node (11) at (121.75bp,698.22bp) [draw,circle] {11};
  \node (12) at (121.75bp,601.72bp) [draw,circle] {12};
  \node (13) at (121.75bp,505.23bp) [draw,circle] {13};
  \node (14) at (121.75bp,408.73bp) [draw,circle] {14};
  \node (15) at (22.748bp,312.24bp) [draw,circle] {15};
  \node (19) at (220.75bp,312.24bp) [draw,circle] {19};
  \node (16) at (22.748bp,215.74bp) [draw,circle] {16};
  \node (17) at (22.748bp,119.24bp) [draw,circle] {17};
  \node (18) at (22.748bp,22.748bp) [draw,circle] {18};
  \node (20) at (220.75bp,215.74bp) [draw,circle] {20};
  \node (21) at (220.75bp,119.24bp) [draw,circle] {21};
  \draw [->] (0) ..controls (121.75bp,1640.0bp) and (121.75bp,1625.1bp)  .. (1);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (181.25bp,1626.0bp) node {timer\_enable 0/τ};
  \draw [->] (1) ..controls (121.75bp,1553.0bp) and (121.75bp,1538.1bp)  .. (2);
  \draw (168.25bp,1539.0bp) node {mov \#0, r8/τ};
  \draw [->] (2) ..controls (121.75bp,1466.0bp) and (121.75bp,1451.1bp)  .. (3);
  \draw (194.25bp,1452.0bp) node {mov \#0, \&reti\_cnt/τ};
  \draw [->] (3) ..controls (121.75bp,1379.0bp) and (121.75bp,1364.1bp)  .. (4);
  \draw (150.75bp,1365.0bp) node {create/τ};
  \draw [->] (4) ..controls (121.75bp,1292.0bp) and (121.75bp,1277.1bp)  .. (5);
  \draw (204.25bp,1278.0bp) node {jin enclave\_start/JmpIn};
  \draw [->] (5) ..controls (121.75bp,1205.0bp) and (121.75bp,1190.1bp)  .. (6);
  \draw (242.25bp,1191.0bp) node {mov \#0, \&secret\_data\_start/Time};
  \draw [->] (6) ..controls (121.75bp,1118.0bp) and (121.75bp,1103.1bp)  .. (7);
  \draw (176.75bp,1104.0bp) node {IRQ/HandleIRQ};
  \draw [->] (7) ..controls (121.75bp,1031.0bp) and (121.75bp,1016.1bp)  .. (8);
  \draw (151.75bp,1017.0bp) node {reti/Reti};
  \draw [->] (8) ..controls (121.75bp,944.05bp) and (121.75bp,929.13bp)  .. (9);
  \draw (240.75bp,929.96bp) node {add \#1, \&secret\_data\_start/Time};
  \draw [->] (9) ..controls (121.75bp,857.13bp) and (121.75bp,842.47bp)  .. (10);
  \draw (239.75bp,842.96bp) node {mov \&secret\_data\_start, r4/Time};
  \draw [->] (10) ..controls (121.75bp,759.79bp) and (121.75bp,745.49bp)  .. (11);
  \draw (201.75bp,746.47bp) node {br \#enclave\_end/Time};
  \draw [->] (11) ..controls (121.75bp,663.29bp) and (121.75bp,649.0bp)  .. (12);
  \draw (210.75bp,649.97bp) node {br \#enclave\_end/JmpOut};
  \draw [->] (12) ..controls (121.75bp,566.8bp) and (121.75bp,552.5bp)  .. (13);
  \draw (194.25bp,553.48bp) node {cmp \#0, \&reti\_cnt/τ};
  \draw [->] (13) ..controls (121.75bp,470.3bp) and (121.75bp,456.01bp)  .. (14);
  \draw (194.25bp,456.98bp) node {mov \#1, \&reti\_cnt/τ};
  \draw [->] (14) ..controls (75.359bp,401.91bp) and (40.588bp,392.5bp)  .. (23.748bp,367.98bp) .. controls (19.459bp,361.74bp) and (17.743bp,354.08bp)  .. (15);
  \draw (111.25bp,360.48bp) node {zthen\_else reti, nop/Reti};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (14) ..controls (160.69bp,395.02bp) and (183.87bp,384.34bp)  .. (198.75bp,367.98bp) .. controls (204.48bp,361.68bp) and (208.81bp,353.69bp)  .. (19);
  \definecolor{strokecol}{rgb}{0.0,0.14,0.4};
  \pgfsetstrokecolor{strokecol}
  \draw (284.75bp,360.48bp) node {zthen\_else nop, nop/τ};
  \draw [->] (15) ..controls (22.748bp,277.31bp) and (22.748bp,263.01bp)  .. (16);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (99.248bp,263.99bp) node {zthen\_else reti, nop/τ};
  \draw [->] (16) ..controls (22.748bp,180.81bp) and (22.748bp,166.52bp)  .. (17);
  \draw (69.248bp,167.49bp) node {cmp \#2, r4/τ};
  \draw [->] (17) ..controls (22.748bp,84.317bp) and (22.748bp,70.022bp)  .. (18);
  \draw (62.248bp,70.996bp) node {rst\_nz/Halt};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (19) ..controls (220.75bp,277.31bp) and (220.75bp,263.01bp)  .. (20);
  \definecolor{strokecol}{rgb}{0.0,0.14,0.4};
  \pgfsetstrokecolor{strokecol}
  \draw (267.25bp,263.99bp) node {cmp \#2, r4/τ};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (20) ..controls (220.75bp,180.81bp) and (220.75bp,166.52bp)  .. (21);
  \draw (265.25bp,167.49bp) node {rst\_nz/Reset};
%
\end{tikzpicture}



==> witnesses/ef753b6-b4.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (0) at (170.75bp,1128.5bp) [draw,circle] {0};
  \node (1) at (170.75bp,1041.5bp) [draw,circle] {1};
  \node (2) at (170.75bp,954.47bp) [draw,circle] {2};
  \node (3) at (170.75bp,867.47bp) [draw,circle] {3};
  \node (4) at (170.75bp,780.47bp) [draw,circle] {4};
  \node (5) at (170.75bp,693.47bp) [draw,circle] {5};
  \node (6) at (58.748bp,601.72bp) [draw,circle] {6};
  \node (13) at (278.75bp,601.72bp) [draw,circle] {13};
  \node (7) at (22.748bp,505.23bp) [draw,circle] {7};
  \node (8) at (22.748bp,408.73bp) [draw,circle] {8};
  \node (9) at (22.748bp,312.24bp) [draw,circle] {9};
  \node (10) at (22.748bp,215.74bp) [draw,circle] {10};
  \node (11) at (22.748bp,119.24bp) [draw,circle] {11};
  \node (12) at (22.748bp,22.748bp) [draw,circle] {12};
  \node (14) at (283.75bp,505.23bp) [draw,circle] {14};
  \node (15) at (283.75bp,408.73bp) [draw,circle] {15};
  \node (16) at (283.75bp,312.24bp) [draw,circle] {16};
  \node (17) at (283.75bp,215.74bp) [draw,circle] {17};
  \node (18) at (283.75bp,119.24bp) [draw,circle] {18};
  \draw [->] (0) ..controls (170.75bp,1099.1bp) and (170.75bp,1084.1bp)  .. (1);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (230.25bp,1085.0bp) node {timer\_enable 0/τ};
  \draw [->] (1) ..controls (170.75bp,1012.1bp) and (170.75bp,997.14bp)  .. (2);
  \draw (199.75bp,997.97bp) node {create/τ};
  \draw [->] (2) ..controls (170.75bp,925.05bp) and (170.75bp,910.14bp)  .. (3);
  \draw (253.25bp,910.97bp) node {jin enclave\_start/JmpIn};
  \draw [->] (3) ..controls (170.75bp,838.05bp) and (170.75bp,823.14bp)  .. (4);
  \draw (289.75bp,823.97bp) node {add \#1, \&secret\_data\_start/Time};
  \draw [->] (4) ..controls (170.75bp,751.05bp) and (170.75bp,736.14bp)  .. (5);
  \draw (225.75bp,736.97bp) node {IRQ/HandleIRQ};
  \draw [->] (5) ..controls (131.58bp,687.14bp) and (97.15bp,678.68bp)  .. (76.748bp,657.47bp) .. controls (69.844bp,650.29bp) and (65.588bp,640.42bp)  .. (6);
  \draw (159.25bp,649.97bp) node {jin enclave\_start/JmpIn};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (5) ..controls (204.57bp,682.3bp) and (228.97bp,672.56bp)  .. (245.75bp,657.47bp) .. controls (253.28bp,650.7bp) and (259.64bp,641.79bp)  .. (13);
  \definecolor{strokecol}{rgb}{0.0,0.14,0.4};
  \pgfsetstrokecolor{strokecol}
  \draw (288.75bp,649.97bp) node {reti/Reti};
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->] (6) ..controls (47.19bp,578.17bp) and (42.985bp,569.24bp)  .. (39.748bp,560.98bp) .. controls (36.314bp,552.21bp) and (33.097bp,542.45bp)  .. (7);
  \definecolor{strokecol}{rgb}{0.64,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (158.75bp,553.48bp) node {add \#1, \&secret\_data\_start/Time};
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->] (7) ..controls (22.748bp,473.31bp) and (22.748bp,454.12bp)  .. (8);
  \draw (140.75bp,456.98bp) node {mov \&secret\_data\_start, r4/Time};
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->] (8) ..controls (22.748bp,376.81bp) and (22.748bp,357.62bp)  .. (9);
  \draw (102.75bp,360.48bp) node {br \#enclave\_end/Time};
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->] (9) ..controls (22.748bp,281.71bp) and (22.748bp,265.0bp)  .. (10);
  \draw (111.75bp,263.99bp) node {br \#enclave\_end/JmpOut};
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->] (10) ..controls (22.748bp,180.81bp) and (22.748bp,166.52bp)  .. (11);
  \draw (69.248bp,167.49bp) node {cmp \#2, r4/τ};
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->] (11) ..controls (22.748bp,84.317bp) and (22.748bp,70.022bp)  .. (12);
  \draw (62.248bp,70.996bp) node {rst\_nz/Halt};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (13) ..controls (280.54bp,566.8bp) and (281.3bp,552.5bp)  .. (14);
  \definecolor{strokecol}{rgb}{0.0,0.14,0.4};
  \pgfsetstrokecolor{strokecol}
  \draw (399.75bp,553.48bp) node {mov \&secret\_data\_start, r4/Time};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (14) ..controls (283.75bp,470.3bp) and (283.75bp,456.01bp)  .. (15);
  \draw (363.75bp,456.98bp) node {br \#enclave\_end/Time};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (15) ..controls (283.75bp,373.8bp) and (283.75bp,359.51bp)  .. (16);
  \draw (372.75bp,360.48bp) node {br \#enclave\_end/JmpOut};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (16) ..controls (283.75bp,277.31bp) and (283.75bp,263.01bp)  .. (17);
  \draw (330.25bp,263.99bp) node {cmp \#2, r4/τ};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (17) ..controls (283.75bp,180.81bp) and (283.75bp,166.52bp)  .. (18);
  \draw (328.25bp,167.49bp) node {rst\_nz/Reset};
%
\end{tikzpicture}



==> witnesses/ef753b6-b6.tex <==
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (0) at (302.75bp,982.96bp) [draw,circle] {0};
  \node (1) at (238.75bp,891.21bp) [draw,circle] {1};
  \node (11) at (364.75bp,891.21bp) [draw,circle] {11};
  \node (2) at (205.75bp,794.72bp) [draw,circle] {2};
  \node (3) at (158.75bp,698.22bp) [draw,circle] {3};
  \node (4) at (146.75bp,601.72bp) [draw,circle] {4};
  \node (5) at (98.748bp,505.23bp) [draw,circle] {5};
  \node (6) at (35.748bp,408.73bp) [draw,circle] {6};
  \node (7) at (31.748bp,312.24bp) [draw,circle] {7};
  \node (8) at (22.748bp,215.74bp) [draw,circle] {8};
  \node (9) at (22.748bp,119.24bp) [draw,circle] {9};
  \node (10) at (22.748bp,22.748bp) [draw,circle] {10};
  \node (12) at (366.75bp,794.72bp) [draw,circle] {12};
  \node (13) at (367.75bp,698.22bp) [draw,circle] {13};
  \node (14) at (367.75bp,601.72bp) [draw,circle] {14};
  \node (15) at (367.75bp,505.23bp) [draw,circle] {15};
  \node (16) at (369.75bp,408.73bp) [draw,circle] {16};
  \node (17) at (371.75bp,312.24bp) [draw,circle] {17};
  \node (18) at (373.75bp,215.74bp) [draw,circle] {18};
  \node (19) at (373.75bp,119.24bp) [draw,circle] {19};
  \node (20) at (373.75bp,22.748bp) [draw,circle] {20};
  \definecolor{strokered}{rgb}{1.0,0.0,0.0};
  \definecolor{strokeblue}{rgb}{0.0,0.0,1.0};
  \definecolor{strokeblack}{rgb}{0.0,0.0,0.0};
  \draw [strokered,->,thick,dotted] (0) ..controls (272.04bp,971.03bp) and (254.12bp,961.63bp)  .. (244.75bp,946.96bp) .. controls (239.81bp,939.23bp) and (237.73bp,929.6bp)  .. (1);
  \draw (291.25bp,939.46bp) node {\texttt{mov \#0, r8}/$\tau$};
  \definecolor{strokeblue}{rgb}{0.0,0.0,1.0};
  \draw [strokeblue,->,dashed,thick] (0) ..controls (325.25bp,965.2bp) and (335.0bp,956.45bp)  .. (341.75bp,946.96bp) .. controls (346.62bp,940.11bp) and (350.73bp,932.07bp)  .. (1);
  \draw (397.25bp,939.46bp) node {\texttt{mov \#1, r8}/$\tau$};
  \draw [->] (1) ..controls (228.08bp,859.66bp) and (220.9bp,839.1bp)  .. (2);
  \definecolor{strokecol}{rgb}{1.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (253.75bp,842.96bp) node {\texttt{create}/$\tau$};
  \draw [->] (2) ..controls (190.96bp,771.96bp) and (185.19bp,762.68bp)  .. (180.75bp,753.97bp) .. controls (176.23bp,745.11bp) and (171.98bp,735.11bp)  .. (3);
  \draw (272.25bp,746.47bp) node {\texttt{mov \#42, \&DMEM\_210}/$\tau$};
  \draw [->] (3) ..controls (154.82bp,666.3bp) and (152.38bp,647.11bp)  .. (4);
  \draw (236.25bp,649.97bp) node {\texttt{jin enclave\_start}/\mi{JmpIn}};
  \draw [->] (4) ..controls (131.46bp,570.62bp) and (120.35bp,548.76bp)  .. (5);
  \draw (186.25bp,553.48bp) node {\texttt{cmp \#0, r8}/\mi{Time}};
  \draw [->] (5) ..controls (74.767bp,486.95bp) and (62.594bp,476.32bp)  .. (54.748bp,464.48bp) .. controls (49.357bp,456.34bp) and (45.323bp,446.51bp)  .. (6);
  \draw (209.75bp,456.98bp) node {\texttt{zero\_or\_nop mov \#1, \&DMEM\_210, 5}/\mi{Time}};
  \draw [->] (6) ..controls (34.439bp,376.81bp) and (33.627bp,357.62bp)  .. (7);
  \draw (189.75bp,360.48bp) node {\texttt{zero\_or\_nop mov \#1, \&DMEM\_210, 5}/\mi{Time}};
  \draw [->] (7) ..controls (28.803bp,280.32bp) and (26.975bp,261.12bp)  .. (8);
  \draw (192.75bp,263.99bp) node {\texttt{zero\_or\_nop mov \#1, \&DMEM\_210, 5}/\mi{JmpOut}};
  \draw [->] (8) ..controls (22.748bp,183.82bp) and (22.748bp,164.63bp)  .. (9);
  \draw (109.75bp,167.49bp) node {\texttt{cmp \#1, \&DMEM\_210}/$\tau$};
  \draw [->] (9) ..controls (22.748bp,88.72bp) and (22.748bp,72.012bp)  .. (10);
  \draw (62.248bp,70.996bp) node {\texttt{rst\_nz}/\mi{Halt}};
  \definecolor{strokecolor}{rgb}{0.0,0.0,1.0};
  \draw [strokecolor,->,dashed] (11) ..controls (365.47bp,856.28bp) and (365.77bp,841.99bp)  .. (12);
  \definecolor{strokecol}{rgb}{0.0,0.0,1.0};
  \pgfsetstrokecolor{strokecol}
  \draw (395.75bp,842.96bp) node {\texttt{create}/$\tau$};
  \definecolor{strokecolor}{rgb}{0.0,0.0,1.0};
  \draw [strokecolor,->,dashed] (12) ..controls (367.11bp,759.79bp) and (367.26bp,745.49bp)  .. (13);
  \draw (459.25bp,746.47bp) node {\texttt{mov \#42, \&DMEM\_210}/$\tau$};
  \definecolor{strokecolor}{rgb}{0.0,0.0,1.0};
  \draw [strokecolor,->,dashed] (13) ..controls (367.75bp,663.29bp) and (367.75bp,649.0bp)  .. (14);
  \draw (450.25bp,649.97bp) node {\texttt{jin enclave\_start}/\mi{JmpIn}};
  \definecolor{strokecolor}{rgb}{0.0,0.0,1.0};
  \draw [strokecolor,->,dashed] (14) ..controls (367.75bp,566.8bp) and (367.75bp,552.5bp)  .. (15);
  \draw (428.25bp,553.48bp) node {\texttt{cmp \#0, r8}/\mi{Time}};
  \definecolor{strokecolor}{rgb}{0.0,0.0,1.0};
  \draw [strokecolor,->,dashed] (15) ..controls (368.47bp,470.3bp) and (368.77bp,456.01bp)  .. (16);
  \draw (523.75bp,456.98bp) node {\texttt{zero\_or\_nop mov \#1, \&DMEM\_210, 5}/\mi{Time}};
  \definecolor{strokecolor}{rgb}{0.0,0.0,1.0};
  \draw [strokecolor,->,dashed] (16) ..controls (370.47bp,373.8bp) and (370.77bp,359.51bp)  .. (17);
  \draw (525.75bp,360.48bp) node {\texttt{zero\_or\_nop mov \#1, \&DMEM\_210, 5}/\mi{Time}};
  \definecolor{strokecolor}{rgb}{0.0,0.0,1.0};
  \draw [strokecolor,->,dashed] (17) ..controls (372.47bp,277.31bp) and (372.77bp,263.01bp)  .. (18);
  \draw (536.75bp,263.99bp) node {\texttt{zero\_or\_nop mov \#1, \&DMEM\_210, 5}/\mi{JmpOut}};
  \definecolor{strokecolor}{rgb}{0.0,0.0,1.0};
  \draw [strokecolor,->,dashed] (18) ..controls (373.75bp,180.81bp) and (373.75bp,166.52bp)  .. (19);
  \draw (460.75bp,167.49bp) node {\texttt{cmp \#1, \&DMEM\_210}/$\tau$};
  \definecolor{strokecolor}{rgb}{0.0,0.0,1.0};
  \draw [strokecolor,->,dashed] (19) ..controls (373.75bp,84.317bp) and (373.75bp,70.022bp)  .. (20);
  \draw (418.25bp,70.996bp) node {\texttt{rst\_nz}/\mi{Reset}};
%
\end{tikzpicture}
}


==> witnesses/ef753b6-b7.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (0) at (149.75bp,1359.4bp) [draw,circle] {0};
  \node (1) at (149.75bp,1272.4bp) [draw,circle] {1};
  \node (2) at (80.748bp,1180.7bp) [draw,circle] {2};
  \node (15) at (216.75bp,1180.7bp) [draw,circle] {15};
  \node (3) at (55.748bp,1084.2bp) [draw,circle] {3};
  \node (4) at (46.748bp,987.71bp) [draw,circle] {4};
  \node (5) at (32.748bp,891.21bp) [draw,circle] {5};
  \node (6) at (28.748bp,794.72bp) [draw,circle] {6};
  \node (7) at (22.748bp,698.22bp) [draw,circle] {7};
  \node (8) at (22.748bp,601.72bp) [draw,circle] {8};
  \node (9) at (22.748bp,505.23bp) [draw,circle] {9};
  \node (10) at (22.748bp,408.73bp) [draw,circle] {10};
  \node (11) at (22.748bp,312.24bp) [draw,circle] {11};
  \node (12) at (22.748bp,215.74bp) [draw,circle] {12};
  \node (13) at (22.748bp,119.24bp) [draw,circle] {13};
  \node (14) at (22.748bp,22.748bp) [draw,circle] {14};
  \node (16) at (220.75bp,1084.2bp) [draw,circle] {16};
  \node (17) at (220.75bp,987.71bp) [draw,circle] {17};
  \node (18) at (221.75bp,891.21bp) [draw,circle] {18};
  \node (19) at (221.75bp,794.72bp) [draw,circle] {19};
  \node (20) at (222.75bp,698.22bp) [draw,circle] {20};
  \node (21) at (222.75bp,601.72bp) [draw,circle] {21};
  \node (22) at (222.75bp,505.23bp) [draw,circle] {22};
  \node (23) at (222.75bp,408.73bp) [draw,circle] {23};
  \node (24) at (222.75bp,312.24bp) [draw,circle] {24};
  \draw [->] (0) ..controls (149.75bp,1330.0bp) and (149.75bp,1315.1bp)  .. (1);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (209.25bp,1315.9bp) node {timer\_enable 4/τ};
  \draw [->] (1) ..controls (119.58bp,1260.2bp) and (101.76bp,1250.7bp)  .. (91.748bp,1236.4bp) .. controls (86.434bp,1228.9bp) and (83.552bp,1219.4bp)  .. (2);
  \draw (138.25bp,1228.9bp) node {mov \#1, r8/τ};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (1) ..controls (171.89bp,1254.4bp) and (181.64bp,1245.7bp)  .. (188.75bp,1236.4bp) .. controls (194.27bp,1229.3bp) and (199.21bp,1220.8bp)  .. (15);
  \definecolor{strokecol}{rgb}{0.0,0.14,0.4};
  \pgfsetstrokecolor{strokecol}
  \draw (245.25bp,1228.9bp) node {mov \#0, r8/τ};
  \draw [->] (2) ..controls (72.617bp,1149.0bp) and (67.361bp,1129.1bp)  .. (3);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (139.25bp,1132.5bp) node {mov \#0, \&irq\_cnt/τ};
  \draw [->] (3) ..controls (52.803bp,1052.3bp) and (50.975bp,1033.1bp)  .. (4);
  \draw (81.748bp,1036.0bp) node {create/τ};
  \draw [->] (4) ..controls (42.207bp,956.06bp) and (39.287bp,936.35bp)  .. (5);
  \draw (123.25bp,939.46bp) node {jin enclave\_start/JmpIn};
  \draw [->] (5) ..controls (31.439bp,859.29bp) and (30.627bp,840.1bp)  .. (6);
  \draw (92.248bp,842.96bp) node {cmp \#0, r8/Time};
  \draw [->] (6) ..controls (26.785bp,762.8bp) and (25.566bp,743.6bp)  .. (7);
  \draw (115.25bp,746.47bp) node {zero\_or\_nop dint, 2/Time};
  \draw [->] (7) ..controls (22.748bp,666.3bp) and (22.748bp,647.11bp)  .. (8);
  \draw (77.748bp,649.97bp) node {IRQ/HandleIRQ};
  \draw [->] (8) ..controls (22.748bp,569.8bp) and (22.748bp,550.61bp)  .. (9);
  \draw (92.248bp,553.48bp) node {mov \#1, \&irq\_cnt/τ};
  \draw [->] (9) ..controls (22.748bp,474.7bp) and (22.748bp,458.0bp)  .. (10);
  \draw (52.748bp,456.98bp) node {reti/Reti};
  \draw [->] (10) ..controls (22.748bp,373.8bp) and (22.748bp,359.51bp)  .. (11);
  \draw (55.748bp,360.48bp) node {reti/Time};
  \draw [->] (11) ..controls (22.748bp,277.31bp) and (22.748bp,263.01bp)  .. (12);
  \draw (65.248bp,263.99bp) node {reti/JmpOut};
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->] (12) ..controls (22.748bp,180.81bp) and (22.748bp,166.52bp)  .. (13);
  \definecolor{strokecol}{rgb}{0.64,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (92.248bp,167.49bp) node {cmp \#0, \&irq\_cnt/τ};
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->] (13) ..controls (22.748bp,84.317bp) and (22.748bp,70.022bp)  .. (14);
  \draw (67.248bp,70.996bp) node {rst\_nz/Reset};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (15) ..controls (218.18bp,1145.8bp) and (218.79bp,1131.5bp)  .. (16);
  \definecolor{strokecol}{rgb}{0.0,0.14,0.4};
  \pgfsetstrokecolor{strokecol}
  \draw (289.25bp,1132.5bp) node {mov \#0, \&irq\_cnt/τ};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (16) ..controls (220.75bp,1049.3bp) and (220.75bp,1035.0bp)  .. (17);
  \draw (249.75bp,1036.0bp) node {create/τ};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (17) ..controls (221.11bp,952.78bp) and (221.26bp,938.49bp)  .. (18);
  \draw (304.25bp,939.46bp) node {jin enclave\_start/JmpIn};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (18) ..controls (221.75bp,856.28bp) and (221.75bp,841.99bp)  .. (19);
  \draw (282.25bp,842.96bp) node {cmp \#0, r8/Time};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (19) ..controls (222.11bp,759.79bp) and (222.26bp,745.49bp)  .. (20);
  \draw (310.25bp,746.47bp) node {zero\_or\_nop dint, 2/Time};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (20) ..controls (222.75bp,663.29bp) and (222.75bp,649.0bp)  .. (21);
  \draw (311.25bp,649.97bp) node {zero\_or\_nop dint, 2/Time};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (21) ..controls (222.75bp,566.8bp) and (222.75bp,552.5bp)  .. (22);
  \draw (320.75bp,553.48bp) node {zero\_or\_nop dint, 2/JmpOut};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (22) ..controls (222.75bp,470.3bp) and (222.75bp,456.01bp)  .. (23);
  \draw (292.25bp,456.98bp) node {cmp \#0, \&irq\_cnt/τ};
  \definecolor{strokecolor}{rgb}{0.0,0.14,0.4};
  \draw [strokecolor,->,dashed] (23) ..controls (222.75bp,373.8bp) and (222.75bp,359.51bp)  .. (24);
  \draw (262.25bp,360.48bp) node {rst\_nz/Halt};
%
\end{tikzpicture}


